Keystone: Proper Refinement Matters More Than Accurate SfM Initialization

Feed-forward reconstruction networks, e.g., VGGT, predict camera poses and dense geometry for a set of images in a single forward pass. They are highly efficient, making them an attractive alternative to classical Structure-from-Motion (SfM) approaches based on local feature matches. However, their camera pose estimates are clearly less accurate than those obtained by feature-based SfM. Recent work has therefore proposed increasingly elaborate pipelines that combine feed-forward predictions with classical SfM. In this paper, we explore a much simpler alternative. We take initial camera poses from any method, such as an off-the-shelf reconstruction network, and iteratively refine them with local feature matches through multiple rounds of triangulation and bundle adjustment. Scenes too large for one forward pass are predicted in two interleaved partitions of overlapping chunks, placed in a common frame by averaging similarity transformations estimated on their shared images, and then refined as a whole. Despite its simplicity, this approach, which we call Keystone, substantially improves feed-forward, classical, and hybrid initializations alike and brings them to nearly the same accuracy. In particular, the noisy poses of feed-forward networks are good enough: starting from them, Keystone outperforms both classical SfM and (significantly more complex) recent hybrid pipelines on standard benchmarks, including challenging settings involving lens distortion and long video sequences. Given its simplicity and strong results, Keystone represents a solid baseline for future research on feed- forward methods for accurate 3D reconstruction and practical SfM systems. Code and Project page: https://keystone-refine.github.io/ .

==> tab/rows/eth3d_scenes_merged.tex <==
% Generated by paper/scripts/make_tables.py
botanical\_garden & \rka{100.0} & \rkc{53.3} & \rkb{86.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 50.0 & 26.7 & 3.3 & 36.7 & \rka{100.0} & 0.0 & \rkc{63.7} & 22.2 & 46.6 & \rkb{64.0} & 37.9 & \rka{69.7} & 61.5 & 6.7 & 3.8 & 1.9 & 3.8 & 51.3 & 5.3 \\
\quad + \method & \rka{100.0} & \rkc{53.3} & \rkb{86.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 89.2 & 30.1 & 66.0 & 89.4 & 89.4 & \rkb{89.7} & 89.4 & \rka{89.8} & 89.5 & 89.5 & 89.1 & 89.3 & \rkc{89.6} \\
boulders & \rka{100.0} & 0.0 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{96.2} & 84.6 & 80.8 & \rkc{88.5} & 80.8 & \rka{100.0} & \rkc{88.5} & \rkc{50.3} & 0.0 & 47.2 & 49.7 & 38.0 & \rka{70.3} & \rkb{60.1} & 10.8 & 17.0 & 7.6 & 13.8 & 42.4 & 26.0 \\
\quad + \method & \rka{100.0} & 0.0 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 86.6 & 0.0 & 86.6 & 86.5 & 86.5 & \rkc{86.8} & 86.6 & 86.6 & 86.3 & 86.4 & 86.1 & \rkb{87.0} & \rka{87.4} \\
bridge & \rkb{72.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 58.2 & \rkc{66.4} & \rka{100.0} & 19.1 & 11.8 & 20.0 & 11.8 & 55.5 & 18.2 & 46.3 & \rkc{77.2} & \rka{77.7} & \rkb{77.4} & 49.1 & 34.4 & 71.3 & 17.8 & 9.9 & 13.1 & 2.0 & 46.9 & 10.2 \\
\quad + \method & \rkc{51.8} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{59.1} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 39.2 & 88.1 & 88.2 & \rkc{88.5} & 88.1 & 43.9 & \rkb{88.6} & 88.0 & 87.3 & 87.8 & 88.4 & \rka{90.1} & \rka{90.1} \\
courtyard & \rkc{76.3} & 26.3 & \rkb{78.9} & \rkb{78.9} & \rkb{78.9} & \rka{92.1} & 68.4 & 50.0 & 15.8 & 50.0 & 73.7 & \rkb{78.9} & 39.5 & \rkc{54.9} & 13.2 & 54.0 & \rkb{55.0} & 44.6 & \rka{63.3} & 53.2 & 24.7 & 16.2 & 17.9 & 34.9 & 41.9 & 21.4 \\
\quad + \method & \rka{100.0} & \rkb{60.5} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 79.8 & 32.6 & 80.1 & 79.8 & 79.9 & 80.0 & 79.8 & 79.4 & \rkc{80.2} & 79.9 & 79.8 & \rkb{84.2} & \rka{88.8} \\
delivery\_area & \rka{100.0} & 18.2 & 45.5 & \rka{100.0} & \rkb{88.6} & \rka{100.0} & \rkb{88.6} & 22.7 & 11.4 & 29.5 & 45.5 & \rkc{70.5} & 22.7 & \rkb{60.4} & 9.7 & 33.7 & \rkc{60.3} & 37.4 & \rka{63.2} & 48.4 & 14.9 & 9.1 & 5.3 & 21.1 & 35.5 & 8.9 \\
\quad + \method & \rka{100.0} & \rkc{36.4} & \rkb{84.1} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{91.9} & 20.5 & 64.5 & \rkb{91.9} & 91.6 & \rkb{91.9} & 91.7 & 91.5 & 91.1 & 91.7 & 91.7 & \rka{92.1} & \rkc{91.8} \\
door & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{78.6} & \rkb{79.4} & 73.5 & 77.3 & 66.9 & 70.2 & \rka{86.4} & 26.2 & 9.8 & 25.5 & 19.6 & 73.4 & 8.9 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 88.0 & 88.0 & \rkc{88.1} & 88.0 & \rka{88.5} & \rkc{88.1} & 87.9 & \rka{88.5} & \rkb{88.2} & \rkc{88.1} & 87.7 & \rka{88.5} & \rkb{88.2} \\
electro & \rkb{97.8} & 91.1 & \rkc{95.6} & \rkb{97.8} & 88.9 & \rka{100.0} & \rkc{95.6} & 68.9 & 55.6 & 55.6 & 64.4 & 91.1 & 64.4 & \rkc{56.1} & 52.4 & 55.0 & \rkb{57.5} & 43.2 & \rka{67.7} & 48.9 & 25.6 & 17.7 & 21.5 & 23.7 & 43.9 & 20.7 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 82.4 & 82.4 & 82.4 & 82.5 & 82.4 & 82.4 & 82.7 & \rkc{82.9} & \rkb{83.1} & 82.4 & 82.6 & 81.6 & \rka{85.9} \\
exhibition\_hall & 39.7 & 2.9 & \rka{100.0} & \rka{100.0} & \rkb{98.5} & \rkc{86.8} & \rka{100.0} & 67.6 & 4.4 & 30.9 & 33.8 & \rkb{98.5} & 1.5 & 10.5 & 0.2 & 24.6 & \rkc{26.6} & 25.2 & \rkb{30.5} & \rkc{26.6} & 5.7 & 0.1 & 2.5 & 3.7 & \rka{30.9} & 0.0 \\
\quad + \method & 39.7 & 4.4 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{89.7} & \rka{100.0} & \rka{100.0} & 75.0 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{80.9} & 21.4 & 0.3 & \rkb{79.9} & \rkc{79.8} & 79.5 & 65.3 & 79.7 & 79.6 & 40.4 & 79.4 & 78.2 & \rka{83.4} & 53.3 \\
facade & 60.5 & \rkc{72.4} & 67.1 & 68.4 & 48.7 & \rkb{75.0} & \rka{78.9} & 2.6 & 25.0 & 14.5 & 18.4 & 61.8 & 43.4 & 71.3 & 55.5 & \rkc{72.6} & \rkb{73.2} & 62.0 & \rka{76.0} & 66.9 & 10.9 & 35.1 & 18.0 & 22.6 & 65.1 & 40.1 \\
\quad + \method & \rka{100.0} & \rkb{84.2} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{88.4} & 65.0 & \rkc{88.3} & \rkb{88.4} & \rkb{88.4} & 88.2 & 88.2 & \rkc{88.3} & \rkc{88.3} & 88.0 & 88.1 & 86.9 & \rka{89.8} \\
kicker & \rka{100.0} & \rkb{96.8} & \rka{100.0} & \rka{100.0} & \rkb{96.8} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{93.5} & \rka{100.0} & \rka{100.0} & \rkb{69.5} & 62.0 & 68.8 & \rkc{69.1} & 45.5 & \rka{72.8} & 64.4 & 37.3 & 51.7 & 28.7 & 35.1 & 38.5 & 51.7 \\
\quad + \method & \rka{100.0} & \rkb{96.8} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 93.3 & 87.6 & \rkc{93.4} & \rkb{93.5} & 93.3 & \rkc{93.4} & 93.3 & \rkb{93.5} & 92.8 & 93.3 & \rka{93.6} & \rkc{93.4} & \rkb{93.5} \\
lecture\_room & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{60.9} & \rka{100.0} & \rka{100.0} & \rkb{95.7} & \rkb{95.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 58.9 & \rkc{62.3} & \rkb{63.1} & \rka{65.9} & 49.9 & 39.1 & 45.4 & 38.5 & 28.3 & 16.5 & 21.7 & 44.0 & 35.5 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{60.9} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 73.5 & 73.5 & 73.6 & \rkc{73.7} & 73.3 & 36.0 & 73.1 & 73.0 & 71.9 & \rkb{73.9} & 73.2 & \rka{76.5} & \rka{76.5} \\
living\_room & 87.7 & 87.7 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{95.4} & \rkb{98.5} & \rkb{98.5} & \rka{100.0} & \rkb{98.5} & 58.8 & 60.3 & \rkc{74.3} & \rkb{75.9} & 51.8 & \rka{78.1} & 62.5 & 28.6 & 26.6 & 24.0 & 26.8 & 36.4 & 35.2 \\
\quad + \method & \rkb{87.7} & \rkb{87.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 68.4 & 68.5 & \rkc{85.2} & 85.1 & 84.6 & 85.0 & 84.8 & 83.9 & 84.4 & 84.0 & 84.2 & \rka{85.6} & \rkb{85.4} \\
lounge & \rkc{70.0} & 60.0 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 60.0 & \rka{100.0} & \rka{100.0} & \rkb{90.0} & \rkb{90.0} & \rka{100.0} & \rka{100.0} & 31.1 & 43.8 & \rkc{63.8} & \rkb{69.0} & 34.2 & \rka{81.6} & 26.7 & 27.4 & 35.9 & 15.9 & 41.1 & 24.1 & 36.0 \\
\quad + \method & \rkc{60.0} & \rkc{60.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{60.0} & \rkb{90.0} & \rkb{90.0} & \rkb{90.0} & \rka{100.0} & \rkb{90.0} & \rka{100.0} & 40.6 & 44.4 & \rkc{68.5} & \rkb{74.5} & 36.0 & \rka{78.6} & 18.6 & 39.2 & 56.6 & 40.7 & 54.7 & 45.3 & 50.1 \\
meadow & 66.7 & \rka{93.3} & \rka{93.3} & \rka{93.3} & 60.0 & \rkb{80.0} & 53.3 & 53.3 & 40.0 & \rkc{73.3} & \rkb{80.0} & 60.0 & 46.7 & 35.8 & \rka{66.9} & \rkb{66.3} & \rkc{62.8} & 30.9 & 61.0 & 45.0 & 35.9 & 21.6 & 32.4 & 52.6 & 31.7 & 38.5 \\
\quad + \method & \rkb{66.7} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & \rka{93.3} & 43.9 & 80.0 & \rkc{80.2} & \rkc{80.2} & 78.1 & 77.9 & 76.4 & 76.9 & 79.9 & 76.2 & 78.1 & \rka{80.8} & \rkb{80.4} \\
observatory & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{96.3} & 3.7 & 25.9 & \rkc{77.8} & \rka{100.0} & 0.0 & 44.3 & \rkc{46.3} & 44.8 & \rkb{47.2} & 31.4 & 44.1 & 38.5 & 17.6 & 1.2 & 7.4 & 10.1 & \rka{60.5} & 1.0 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 59.8 & 59.7 & 59.9 & 59.8 & \rkc{60.7} & 60.6 & 60.1 & 60.3 & 60.2 & 60.1 & 60.3 & \rkb{62.3} & \rka{65.9} \\
office & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 84.6 & \rka{100.0} & \rkb{96.2} & 88.5 & 57.7 & 88.5 & \rkc{92.3} & 73.1 & 80.8 & \rka{30.2} & 29.3 & 28.9 & \rkc{29.6} & 17.4 & \rkb{29.9} & 27.6 & 19.0 & 10.7 & 20.0 & 18.5 & 18.0 & 21.5 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{58.9} & 58.0 & 57.5 & \rkb{58.6} & 56.7 & 57.5 & 56.8 & 56.7 & 56.6 & 57.0 & 55.8 & \rkc{58.5} & 57.3 \\
old\_computer & 53.7 & 33.3 & \rkb{98.1} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{98.1} & 14.8 & \rkc{77.8} & \rkc{77.8} & \rka{100.0} & 0.0 & 23.0 & 14.4 & \rkc{41.3} & \rkb{44.9} & 27.0 & \rka{48.8} & 36.8 & 13.1 & 0.8 & 7.3 & 8.8 & 30.0 & 0.0 \\
\quad + \method & \rkb{53.7} & \rkc{33.3} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 33.9 & 18.8 & 79.1 & 79.3 & \rkb{79.6} & \rkc{79.4} & 79.2 & \rkb{79.6} & 78.1 & 78.8 & 77.7 & \rka{79.8} & 74.9 \\
pipes & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{92.9} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{92.9} & \rka{100.0} & \rka{100.0} & \rkc{71.4} & \rka{100.0} & \rkc{61.7} & \rkb{62.9} & 60.2 & 60.6 & 22.2 & \rka{63.5} & 46.4 & 30.5 & 9.7 & 29.8 & 38.3 & 18.6 & 29.1 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 85.9 & 86.0 & 85.9 & \rkc{86.2} & 85.2 & 85.8 & \rkc{86.2} & 85.5 & 85.1 & 85.6 & 85.3 & \rka{87.3} & \rkb{87.1} \\
playground & \rka{100.0} & 42.1 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{84.2} & 73.7 & 78.9 & \rkb{92.1} & \rka{100.0} & 71.1 & 69.0 & 19.0 & \rkb{69.7} & \rkb{69.7} & 59.4 & \rka{83.5} & \rkc{69.3} & 18.5 & 8.9 & 17.1 & 19.5 & 46.5 & 10.5 \\
\quad + \method & \rka{100.0} & \rkb{44.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{85.4} & 24.4 & \rkc{85.4} & \rkc{85.4} & \rkb{85.5} & 85.3 & \rkc{85.4} & 85.3 & 85.1 & 85.3 & \rkb{85.5} & 82.9 & \rka{89.4} \\
relief & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 35.5 & 32.3 & \rkb{64.5} & \rkc{54.8} & \rka{100.0} & 22.6 & 61.8 & \rkb{64.1} & \rkc{63.1} & 62.6 & 44.6 & \rka{67.7} & 58.6 & 4.9 & 6.2 & 4.6 & 3.6 & 51.4 & 6.3 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 92.5 & 92.5 & 92.7 & 92.7 & 92.7 & 92.8 & 92.9 & \rkc{93.2} & 92.9 & 92.9 & 92.7 & \rkb{93.4} & \rka{93.7} \\
relief\_2 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 64.5 & \rka{100.0} & \rka{100.0} & \rkc{71.0} & 41.9 & 45.2 & \rkb{77.4} & 54.8 & 51.6 & \rkb{57.8} & \rkc{57.4} & 56.9 & 57.0 & 19.0 & \rka{66.0} & 56.5 & 3.5 & 5.0 & 0.8 & 3.0 & 25.3 & 4.5 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 90.5 & 90.5 & 90.6 & 90.5 & \rkc{90.8} & 90.6 & 90.5 & \rka{91.3} & 89.9 & \rkb{90.9} & 90.7 & \rkc{90.8} & \rkb{90.9} \\
statue & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{27.3} & \rka{100.0} & \rkb{36.4} & \rka{100.0} & \rka{100.0} & 62.2 & \rkc{63.8} & 63.1 & 63.2 & 56.9 & \rkb{68.6} & 59.4 & 19.3 & 1.4 & 20.1 & 4.1 & \rka{73.9} & 39.8 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 86.3 & 86.9 & 88.9 & 88.7 & 86.4 & 86.3 & 89.3 & 85.9 & \rkc{89.5} & 87.6 & 88.3 & \rkb{96.1} & \rka{96.2} \\
terrace & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkc{91.3} & \rkb{95.7} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 78.3 & 55.5 & \rkb{57.6} & 55.9 & \rkc{57.3} & 49.4 & \rka{71.1} & \rkb{57.6} & 43.8 & 28.0 & 37.1 & 41.2 & 44.3 & 29.4 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 89.4 & 89.3 & 89.2 & 89.2 & 89.4 & \rkc{89.5} & 89.2 & 89.2 & 88.9 & 89.1 & 89.3 & \rkb{91.0} & \rka{93.0} \\
terrace\_2 & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 78.0 & \rkc{80.0} & 79.2 & 79.5 & 59.6 & \rka{80.8} & 79.2 & 48.4 & 33.7 & 48.4 & 50.9 & \rkb{80.1} & 49.6 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & 87.0 & 87.0 & 87.0 & 87.0 & \rkc{87.2} & 86.9 & 87.0 & 86.9 & 86.9 & 86.8 & 86.7 & \rkb{89.8} & \rka{90.2} \\
terrains & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{95.2} & 38.1 & 26.2 & 78.6 & \rka{100.0} & \rkc{90.5} & \rkc{68.4} & \rkb{69.2} & 67.6 & \rka{69.7} & 50.1 & 63.2 & 51.1 & 20.9 & 6.6 & 4.1 & 15.7 & 26.7 & 18.1 \\
\quad + \method & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rka{100.0} & \rkb{97.6} & \rka{100.0} & \rka{100.0} & \rkc{71.4} & 9.5 & 0.0 & 57.1 & \rka{100.0} & 52.4 & \rka{64.3} & \rkb{64.1} & \rkc{61.7} & \rkb{64.1} & 46.0 & 59.1 & 47.6 & 42.0 & 29.4 & 29.0 & 33.8 & 36.8 & 35.3 \\
\midrule
\textbf{Average} & 89.0 & 75.1 & \rkb{94.6} & \rka{97.5} & 90.4 & \rkc{94.4} & 93.5 & 75.2 & 53.6 & 66.3 & 72.6 & 88.6 & 60.7 & 54.3 & 46.8 & \rkc{58.1} & \rkb{61.0} & 42.1 & \rka{62.6} & 53.9 & 22.0 & 15.8 & 17.1 & 21.4 & 43.2 & 21.9 \\
\quad + \method & 90.4 & 78.2 & 98.6 & \rka{99.7} & \rkb{99.6} & 96.1 & 98.1 & 98.2 & 94.7 & 95.3 & 98.0 & \rkc{99.3} & 97.1 & 72.8 & 60.7 & 80.1 & \rka{82.5} & 80.0 & 78.4 & 79.4 & 79.9 & 78.5 & 79.4 & 80.1 & \rkb{81.3} & \rkc{81.0} \\


==> tab/rows/partitions.tex <==
\textbf{2} & \textbf{16.8} & \textbf{29.3} & \textbf{72.8} & \textbf{75.5} & \textbf{596} & \textbf{1.5} & \textbf{22.5} & \textbf{24.0} \\
3 & 20.2 & 32.5 & 76.8 & 79.4 & 862 & 2.1 & 20.2 & 22.3 \\
4 & 21.3 & 36.7 & 70.9 & 73.6 & 1{,}130 & 2.8 & 28.6 & 31.4 \\
5 & 21.3 & 36.8 & 71.8 & 73.8 & 1{,}411 & 3.5 & 18.0 & 21.5 \\

